All for One, and One for All: UrbanSyn Dataset, the third Musketeer of Synthetic Driving Scenes

We introduce UrbanSyn, a photorealistic dataset acquired through semi-procedurally generated synthetic urban driving scenarios. Developed using high-quality geometry and materials, UrbanSyn provides pixel-level ground truth, including depth, semantic segmentation, and instance segmentation with object bounding boxes and occlusion degree. It complements GTAV and Synscapes datasets to form what we coin as the 'Three Musketeers'. We demonstrate the value of the Three Musketeers in unsupervised domain adaptation for image semantic segmentation. Results on real-world datasets, Cityscapes, Mapillary Vistas, and BDD100K, establish new benchmarks, largely attributed to UrbanSyn. We make UrbanSyn openly and freely accessible (www.urbansyn.org).

==> tables/results_bbdd.tex <==
\begin{table*}[t]
\vspace{-4mm}
\caption{Analogous to Table \ref{tab:cityscapes_quantitative} but for BDD100K as target. (*) The bad results on the class Train are due to inconsistencies in the validation set labeling as we will illustrate in Section \ref{ssec:errorshumanlabels}.}
\label{tab:bdd_quantitative}
\centering
\setlength{\tabcolsep}{0.9mm} 
\scalebox{0.72}[0.72]{
\begin{tabular}{l|c|c|ccccccccccccccccccc!{\vrule width 1pt}c!{\vrule width 1pt}}

Method & Source & & \rotatebox[origin=c]{90}{\footnotesize Road} & \rotatebox[origin=c]{90}{\footnotesize Sidewalk} & \rotatebox[origin=c]{90}{\footnotesize Building} & \rotatebox[origin=c]{90}{\footnotesize Wall} & \rotatebox[origin=c]{90}{\footnotesize Fence} & \rotatebox[origin=c]{90}{\footnotesize Pole} & \rotatebox[origin=c]{90}{\footnotesize Traffic Light} & \rotatebox[origin=c]{90}{\footnotesize Traffic Sign} & \rotatebox[origin=c]{90}{\footnotesize Vegetation} & \rotatebox[origin=c]{90}{\footnotesize Terrain} & \rotatebox[origin=c]{90}{\footnotesize Sky} & \rotatebox[origin=c]{90}{\footnotesize Person} & \rotatebox[origin=c]{90}{\footnotesize Rider} & \rotatebox[origin=c]{90}{\footnotesize Car} & \rotatebox[origin=c]{90}{\footnotesize Truck} & \rotatebox[origin=c]{90}{\footnotesize Bus} & \rotatebox[origin=c]{90}{{\footnotesize Train}*} & \rotatebox[origin=c]{90}{\footnotesize Motorbike} & \rotatebox[origin=c]{90}{\footnotesize Bike} & mIoU  \\

\noalign{\hrule height 2pt}

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV}  & mean & $76.2$  & $25.9$  & $\bbest{75.8}$  & $\bbest{8.8}$  & $\bbest{35.0}$  & $39.2$  & $\bbest{42.0}$  & $24.8$  & $72.2$  & $\bbest{35.1}$  & $\bbest{88.3}$  & $\bbest{55.6}$  & $\bbest{26.2}$  & $74.8$  & $\bbest{26.7}$  & $13.2$  & $\gbbest{0.0}$  & $\bbest{41.0}$  & $21.9$  & $\bbest{41.2}$ \\ 
& & std & $\stdx{2.9}$  & $\stdx{0.6}$  & $\stdx{0.4}$  & $\stdx{3.1}$  & $\stdx{1.7}$  & $\stdx{0.2}$  & $\stdx{1.2}$  & $\stdx{1.5}$  & $\stdx{1.3}$  & $\stdx{0.7}$  & $\stdx{0.6}$  & $\stdx{0.6}$  & $\stdx{1.6}$  & $\stdx{5.5}$  & $\stdx{1.3}$  & $\stdx{2.6}$  & $\stdx{0.0}$  & $\stdx{1.8}$  & $\stdx{6.7}$  & $\stdx{0.2}$ \\ 

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{Synscapes}  & mean & $79.8$  & $\bbest{29.9}$  & $62.6$  & $2.9$  & $15.8$  & $29.9$  & $27.9$  & ${32.9}$  & $\bbest{73.6}$  & $20.2$  & $86.1$  & $49.4$  & $18.2$  & $72.8$  & $10.3$  & $13.7$  & $\gbbest{0.0}$  & $38.9$  & $\bbest{41.3}$  & $37.2$ \\ 
& & std & $\stdx{2.6}$  & $\stdx{0.6}$  & $\stdx{1.2}$  & $\stdx{0.1}$  & $\stdx{2.7}$  & $\stdx{1.1}$  & $\stdx{0.8}$  & $\stdx{1.1}$  & $\stdx{0.8}$  & $\stdx{2.3}$  & $\stdx{0.8}$  & $\stdx{1.3}$  & $\stdx{1.9}$  & $\stdx{2.3}$  & $\stdx{1.5}$  & $\stdx{3.3}$  & $\stdx{0.0}$  & $\stdx{3.3}$  & $\stdx{3.6}$  & $\stdx{0.3}$ \\ 

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{{\thedataset}}   & mean & $\bbest{86.3}$  & $24.1$  & $63.2$  & $4.6$  & $25.4$  & $\bbest{40.6}$  & $39.8$  & $\bbest{40.1}$  & $65.6$  & $19.7$  & $78.6$  & $45.7$  & $22.6$  & $\bbest{82.7}$  & $21.7$  & $\bbest{51.3}$  & $\gbbest{0.0}$  & $38.6$  & $34.3$  & $\bbest{41.3}$ \\ 
& & std & $\stdx{0.8}$  & $\stdx{3.9}$  & $\stdx{2.3}$  & $\stdx{0.4}$  & $\stdx{5.9}$  & $\stdx{0.3}$  & $\stdx{1.2}$  & $\stdx{1.5}$  & $\stdx{2.2}$  & $\stdx{2.4}$  & $\stdx{1.7}$  & $\stdx{2.6}$  & $\stdx{3.8}$  & $\stdx{0.1}$  & $\stdx{2.2}$  & $\stdx{4.2}$  & $\stdx{0.1}$  & $\stdx{1.6}$  & $\stdx{4.2}$  & $\stdx{0.8}$ \\  \hline

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV+Synscapes}  & mean & $82.4$  & $31.6$  & ${78.7}$  & $\bbest{18.4}$  & $\bbest{38.0}$  & $43.0$  & ${45.1}$  & $30.1$  & $\bbest{76.8}$  & $\bbest{35.8}$  & $\bbest{89.4}$  & $\bbest{61.4}$  & $24.2$  & $76.2$  & $30.5$  & $\bbest{44.9}$  & $\gbbest{0.0}$  & $52.4$  & $50.1$  & $47.8$ \\ 
& & std & $\stdx{3.8}$  & $\stdx{1.2}$  & $\stdx{1.0}$  & $\stdx{1.0}$  & $\stdx{0.8}$  & $\stdx{0.9}$  & $\stdx{1.0}$  & $\stdx{1.6}$  & $\stdx{0.6}$  & $\stdx{0.5}$  & $\stdx{0.6}$  & $\stdx{0.6}$  & $\stdx{2.1}$  & $\stdx{4.0}$  & $\stdx{1.4}$  & $\stdx{11.7}$  & $\stdx{0.0}$  & $\stdx{1.5}$  & $\stdx{3.1}$  & $\stdx{1.2}$ \\

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}   & mean & $\bbest{87.7}$  & $\bbest{37.8}$  & $\bbest{80.1}$  & $\bbest{18.1}$  & $37.0$  & $\bbest{45.5}$  & $\bbest{46.8}$  & $\bbest{42.1}$  & $75.1$  & $\bbest{36.5}$  & $\bbest{89.2}$  & $\bbest{62.0}$  & $\bbest{41.6}$  & $\bbest{82.3}$  & $\bbest{35.0}$  & $\bbest{45.8}$  & $\gbbest{0.0}$  & $\bbest{56.8}$  & $\bbest{59.2}$  & $\bbest{51.5}$ \\ 
& & std & $\stdx{1.4}$  & $\stdx{2.6}$  & $\stdx{0.1}$  & $\stdx{4.1}$  & $\stdx{1.8}$  & $\stdx{0.2}$  & $\stdx{0.6}$  & $\stdx{1.0}$  & $\stdx{1.0}$  & $\stdx{1.6}$  & $\stdx{0.7}$  & $\stdx{1.5}$  & $\stdx{5.3}$  & $\stdx{2.1}$  & $\stdx{1.6}$  & $\stdx{2.9}$  & $\stdx{0.0}$  & $\stdx{0.6}$  & $\stdx{1.2}$  & $\stdx{0.5}$ \\   \hline

 \multirow{2}{*}{HRDA} & \multirow{2}{*}{GTAV}   & mean & $90.0$  & $28.2$  & $\bbest{81.3}$  & $\gbbest{29.9}$  & ${38.6}$  & ${42.6}$  & $\bbest{48.2}$  & $38.6$  & ${80.6}$  & ${41.3}$  & $\bbest{91.3}$  & ${60.5}$  & $\bbest{38.5}$  & $85.2$  & $42.1$  & $65.0$  & $\gbbest{0.0}$  & $43.1$  & $34.1$  & $\bbest{51.5}$ \\  
\UDAbackbone{(DAFormer*)} & & std & $\stdx{0.9}$  & $\stdx{10.8}$  & $\stdx{0.5}$  & $\stdx{2.0}$  & $\stdx{1.0}$  & $\stdx{0.4}$  & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{0.3}$  & $\stdx{2.2}$  & $\stdx{0.2}$  & $\stdx{0.6}$  & $\stdx{3.8}$  & $\stdx{0.5}$  & $\stdx{2.1}$  & $\stdx{3.2}$  & $\stdx{0.0}$  & $\stdx{4.1}$  & $\stdx{2.7}$  & $\stdx{1.2}$ \\ 

\multirow{2}{*}{HRDA} & \multirow{2}{*}{Synscapes}  & mean & $61.5$  & $18.8$  & $78.1$  & $9.0$  & $15.9$  & $38.6$  & $43.4$  & $26.3$  & $79.4$  & $16.3$  & $\bbest{91.3}$  & $58.2$  & $27.5$  & $85.1$  & $25.7$  & $49.1$  & $\gbbest{0.0}$  & $\bbest{46.4}$  & ${51.4}$  & $43.3$ \\ 
\UDAbackbone{(DAFormer*)} & & std & $\stdx{24.6}$  & $\stdx{9.2}$  & $\stdx{1.0}$  & $\stdx{4.6}$  & $\stdx{2.6}$  & $\stdx{1.0}$  & $\stdx{1.4}$  & $\stdx{1.7}$  & $\stdx{0.7}$  & $\stdx{10.6}$  & $\stdx{0.5}$  & $\stdx{2.1}$  & $\stdx{0.9}$  & $\stdx{1.6}$  & $\stdx{9.6}$  & $\stdx{6.4}$  & $\stdx{0.0}$  & $\stdx{2.4}$  & $\stdx{0.6}$  & $\stdx{2.9}$ \\ 

\multirow{2}{*}{HRDA} & \multirow{2}{*}{{\thedataset}}   & mean & $\gbbest{92.1}$  & $\bbest{45.9}$  & $\bbest{81.0}$  & $8.3$  & $\bbest{40.2}$  & $\bbest{43.7}$  & $\bbest{49.1}$  & $\gbbest{53.6}$  & $\bbest{81.7}$  & $\gbbest{42.9}$  & $\bbest{91.4}$  & $\bbest{64.5}$  & $34.4$  & $\gbbest{87.9}$  & $\bbest{45.0}$  & $\bbest{69.2}$  & $\gbbest{0.0}$  & $44.0$  & $\bbest{54.1}$  & $\bbest{54.2}$ \\ 
\UDAbackbone{(DAFormer*)} & & std & $\stdx{0.4}$  & $\stdx{1.1}$  & $\stdx{0.4}$  & $\stdx{3.1}$  & $\stdx{1.3}$  & $\stdx{0.8}$  & $\stdx{0.6}$  & $\stdx{0.5}$  & $\stdx{0.4}$  & $\stdx{2.2}$  & $\stdx{0.3}$  & $\stdx{2.4}$  & $\stdx{7.9}$  & $\stdx{0.3}$  & $\stdx{1.4}$  & $\stdx{1.4}$  & $\stdx{0.0}$  & $\stdx{10.2}$  & $\stdx{0.5}$  & $\stdx{0.8}$ \\    \hline

\multirow{2}{*}{HRDA} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}  & mean & $90.5$  & $\gbbest{56.7}$  & $\gbbest{82.6}$  & $\gbbest{29.3}$  & $\gbbest{41.8}$  & $\gbbest{49.5}$  & $\gbbest{52.5}$  & $52.4$  & $\gbbest{82.7}$  & $\gbbest{43.8}$  & $\gbbest{92.7}$  & $\gbbest{67.0}$  & $\gbbest{47.5}$  & $81.9$  & $\gbbest{49.8}$  & $\gbbest{76.1}$  & $\gbbest{0.0}$  & $\gbbest{55.1}$  & $\gbbest{62.0}$  & $\gbbest{58.6}$ \\ 
\UDAbackbone{(DAFormer*)} & & std & $\stdx{0.5}$  & $\stdx{0.9}$  & $\stdx{0.1}$  & $\stdx{1.1}$  & $\stdx{1.8}$  & $\stdx{0.1}$  & $\stdx{1.1}$  & $\stdx{0.9}$  & $\stdx{0.3}$  & $\stdx{0.6}$  & $\stdx{0.2}$  & $\stdx{1.3}$  & $\stdx{2.5}$  & $\stdx{1.5}$  & $\stdx{1.0}$  & $\stdx{3.1}$  & $\stdx{0.0}$  & $\stdx{1.7}$  & $\stdx{1.0}$  & $\stdx{0.4}$ \\  [-0.35ex] 

\hline

\rowcolor{gray!20}  &  & mean & $95.0$  & $66.1$  & $87.2$  & $34.2$  & $52.7$  & $51.0$  & $56.8$  & $57.4$  & $87.4$  & $53.0$  & $95.8$  & $66.4$  & $29.7$  & $90.7$  & $61.3$  & $81.8$  & $0.0$  & $48.7$  & $52.8$  & $61.5$ \\
\rowcolor{gray!20} \multirow{-2}{*}{SegFormer} & \multirow{-2}{*}{BDD100K (\bbest{reference})} & std & $\stdx{0.1}$  & $\stdx{0.6}$  & $\stdx{0.0}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{0.5}$  & $\stdx{0.3}$  & $\stdx{0.1}$  & $\stdx{1.0}$  & $\stdx{0.2}$  & $\stdx{0.6}$  & $\stdx{12.7}$  & $\stdx{0.5}$  & $\stdx{1.1}$  & $\stdx{2.0}$  & $\stdx{0.0}$  & $\stdx{7.9}$  & $\stdx{3.8}$  & $\stdx{1.2}$ \\ [-0.35ex] 

\specialrule{.14em}{.2em}{.2em}
 &&&&&&&&&&&&&&&&&&&&&&\\[-3ex]




\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{GTAV} & mean & $63.6$  & ${25.9}$  & $59.4$  & $\bbest{6.3}$  & $\bbest{27.6}$  & $32.3$  & $\bbest{36.0}$  & $21.3$  & $66.2$  & $21.1$  & $77.1$  & $\bbest{52.2}$  & $16.9$  & $\bbest{68.2}$  & $18.4$  & $17.9$  & $\gbbest{0.0}$  & $29.0$  & $6.1$  & $34.0$ \\ 
& & std & $\stdx{3.7}$  & $\stdx{1.8}$  & $\stdx{2.5}$  & $\stdx{0.5}$  & $\stdx{2.1}$  & $\stdx{0.8}$  & $\stdx{0.5}$  & $\stdx{1.7}$  & $\stdx{0.6}$  & $\stdx{3.0}$  & $\stdx{2.6}$  & $\stdx{1.3}$  & $\stdx{1.9}$  & $\stdx{1.2}$  & $\stdx{1.0}$  & $\stdx{1.5}$  & $\stdx{0.0}$  & $\stdx{7.3}$  & $\stdx{1.8}$  & $\stdx{0.1}$ \\ 

\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{Synscapes}  & mean & $66.5$  & $21.1$  & $32.9$  & $1.1$  & $5.1$  & $22.3$  & $25.3$  & ${23.2}$  & $61.9$  & $6.5$  & $57.3$  & $47.3$  & ${17.9}$  & $63.3$  & $1.6$  & $5.7$  & $\gbbest{0.0}$  & $30.8$  & $34.0$  & $27.6$ \\ 
& & std & $\stdx{5.4}$  & $\stdx{2.5}$  & $\stdx{3.7}$  & $\stdx{0.5}$  & $\stdx{0.8}$  & $\stdx{2.8}$  & $\stdx{0.9}$  & $\stdx{1.5}$  & $\stdx{3.8}$  & $\stdx{0.4}$  & $\stdx{6.5}$  & $\stdx{3.5}$  & $\stdx{3.4}$  & $\stdx{2.3}$  & $\stdx{0.6}$  & $\stdx{0.5}$  & $\stdx{0.0}$  & $\stdx{2.5}$  & $\stdx{4.2}$  & $\stdx{1.1}$ \\ 

\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{{\thedataset}}  & mean & $\bbest{80.1}$  & $\bbest{29.3}$  & $\bbest{64.8}$  & $3.3$  & $15.8$  & $\bbest{33.6}$  & $31.3$  & $\bbest{33.2}$  & $\bbest{74.1}$  & $\bbest{24.2}$  & $\bbest{79.5}$  & $42.5$  & $\bbest{22.4}$  & $\bbest{68.7}$  & $\bbest{19.6}$  & $\bbest{22.6}$  & $\gbbest{0.0}$  & $\bbest{45.3}$  & $\bbest{50.6}$  & $\bbest{39.0}$ \\
& & std & $\stdx{1.6}$  & $\stdx{1.4}$  & $\stdx{0.8}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{0.4}$  & $\stdx{0.6}$  & $\stdx{0.3}$  & $\stdx{1.6}$  & $\stdx{1.0}$  & $\stdx{7.8}$  & $\stdx{8.0}$  & $\stdx{1.4}$  & $\stdx{1.7}$  & $\stdx{5.2}$  & $\stdx{0.0}$  & $\stdx{0.6}$  & $\stdx{1.2}$  & $\stdx{0.5}$ \\   \hline

\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{GTAV+Synscapes} & mean & $67.2$  & $30.2$  & $74.7$  & $12.9$  & $29.9$  & $\bbest{37.7}$  & $\bbest{39.6}$  & ${27.7}$  & $\bbest{75.0}$  & $25.1$  & $86.5$  & $\bbest{57.9}$  & $\bbest{37.1}$  & $62.0$  & $20.7$  & $25.0$  & $\gbbest{0.1}$  & $\bbest{47.5}$  & $50.5$  & $42.5$ \\ 
& & std & $\stdx{1.3}$  & $\stdx{2.3}$  & $\stdx{0.9}$  & $\stdx{3.0}$  & $\stdx{2.1}$  & $\stdx{2.0}$  & $\stdx{2.5}$  & $\stdx{0.9}$  & $\stdx{0.3}$  & $\stdx{1.6}$  & $\stdx{1.0}$  & $\stdx{1.6}$  & $\stdx{3.4}$  & $\stdx{1.6}$  & $\stdx{0.1}$  & $\stdx{1.6}$  & $\stdx{0.0}$  & $\stdx{1.8}$  & $\stdx{5.2}$  & $\stdx{1.1}$ \\ 

\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}   & mean & $\bbest{78.8}$  & $\bbest{34.7}$  & $\bbest{76.4}$  & $11.2$  & $\bbest{32.6}$  & $36.9$  & $37.0$  & $\bbest{29.5}$  & $\bbest{75.8}$  & $\bbest{33.1}$  & $\bbest{87.7}$  & $56.9$  & $26.5$  & $\bbest{71.2}$  & $\bbest{25.6}$  & $\bbest{45.1}$  & $\gbbest{0.0}$  & $\bbest{47.1}$  & $\bbest{55.8}$  & $\bbest{45.4}$ \\
& & std & $\stdx{0.2}$  & $\stdx{1.5}$  & $\stdx{0.5}$  & $\stdx{1.5}$  & $\stdx{2.1}$  & $\stdx{0.4}$  & $\stdx{0.3}$  & $\stdx{0.4}$  & $\stdx{0.7}$  & $\stdx{0.1}$  & $\stdx{0.5}$  & $\stdx{0.6}$  & $\stdx{2.9}$  & $\stdx{1.5}$  & $\stdx{0.3}$  & $\stdx{2.3}$  & $\stdx{0.0}$  & $\stdx{0.1}$  & $\stdx{1.4}$  & $\stdx{0.5}$ \\  \hline 

\multirow{2}{*}{Co-training} & \multirow{2}{*}{GTAV}    & mean & $82.7$  & $\gbbest{56.0}$  & $\bbest{77.9}$  & $\bbest{20.8}$  & $\bbest{41.7}$  & $36.9$  & $\bbest{34.9}$  & $19.7$  & $74.8$  & $\gbbest{37.4}$  & $87.5$  & $54.8$  & ${40.3}$  & $71.3$  & $27.5$  & $4.5$  & $\gbbest{0.4}$  & $38.4$  & $19.1$  & $43.5$ \\ 
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{1.1}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{1.4}$  & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{0.4}$  & $\stdx{0.3}$  & $\stdx{0.0}$  & $\stdx{0.2}$  & $\stdx{0.9}$  & $\stdx{0.5}$  & $\stdx{0.3}$  & $\stdx{0.6}$  & $\stdx{0.2}$  & $\stdx{0.4}$  & $\stdx{0.5}$  & $\stdx{3.6}$  & $\stdx{0.3}$ \\ 
\multirow{2}{*}{Co-training} & \multirow{2}{*}{Synscapes}   & mean & $\bbest{89.9}$  & $35.5$  & $52.7$  & $1.5$  & $6.9$  & $\bbest{39.5}$  & $32.2$  & $25.9$  & $\gbbest{78.6}$  & $25.5$  & $77.2$  & $\bbest{60.5}$  & $30.2$  & ${85.5}$  & $1.7$  & $29.6$  & $\gbbest{0.0}$  & $\gbbest{50.3}$  & $54.4$  & $40.9$ \\ 
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.4}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.2}$  & $\stdx{0.2}$  & $\stdx{1.1}$  & $\stdx{0.6}$  & $\stdx{0.5}$  & $\stdx{4.5}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{0.0}$  & $\stdx{2.4}$  & $\stdx{0.5}$  & $\stdx{0.3}$ \\
\multirow{2}{*}{Co-training} & \multirow{2}{*}{{\thedataset}}  & mean & $\bbest{90.5}$  & $36.3$  & $76.9$  & $10.0$  & $29.2$  & $31.2$  & $30.1$  & $\bbest{32.3}$  & $74.8$  & $\gbbest{37.7}$  & $\gbbest{88.7}$  & $47.8$  & $\bbest{44.8}$  & $\gbbest{86.7}$  & $\bbest{37.7}$  & $\bbest{65.4}$  & $\gbbest{0.0}$  & $37.1$  & $43.1$  & $\bbest{47.4}$ \\  
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.0}$  & $\stdx{0.9}$  & $\stdx{0.3}$  & $\stdx{0.0}$  & $\stdx{0.8}$  & $\stdx{0.3}$  & $\stdx{0.8}$  & $\stdx{0.7}$  & $\stdx{0.2}$  & $\stdx{0.3}$  & $\stdx{0.1}$  & $\stdx{4.3}$  & $\stdx{1.9}$  & $\stdx{0.1}$  & $\stdx{1.5}$  & $\stdx{2.6}$  & $\stdx{0.0}$  & $\stdx{0.7}$  & $\stdx{1.7}$  & $\stdx{0.3}$ \\ \hline

\multirow{2}{*}{Co-training} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}  & mean & $\gbbest{92.1}$  & $44.4$  & $\gbbest{81.1}$  & $\gbbest{24.2}$  & $\gbbest{44.1}$  & $\gbbest{43.2}$  & $\gbbest{46.6}$  & $\gbbest{40.3}$  & $72.4$  & $36.4$  & $87.0$  & $\gbbest{64.0}$  & $\gbbest{57.7}$  & $\gbbest{87.5}$  & $\gbbest{46.0}$  & $\gbbest{76.9}$  & $\gbbest{0.7}$  & $\gbbest{51.1}$  & $\gbbest{55.7}$  & $\gbbest{55.3}$ \\ 
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.6}$  & $\stdx{0.1}$  & $\stdx{2.2}$  & $\stdx{0.6}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.6}$  & $\stdx{0.1}$  & $\stdx{0.7}$  & $\stdx{1.4}$  & $\stdx{0.0}$  & $\stdx{0.7}$  & $\stdx{0.7}$  & $\stdx{0.2}$  & $\stdx{0.5}$  & $\stdx{0.9}$  & $\stdx{0.1}$ \\  \hline

\rowcolor{gray!20}  &  & mean & ${94.7}$  & ${65.7}$  & ${86.5}$  & ${36.1}$  & ${53.8}$  & ${50.9}$  & ${54.4}$  & ${55.4}$  & ${86.8}$  & ${50.7}$  & ${95.1}$  & ${65.0}$  & ${45.9}$  & ${90.6}$  & ${59.7}$  & ${81.0}$  & ${0.0}$  & ${47.6}$  & $43.4$  & ${61.2}$ \\ 
\rowcolor{gray!20} \multirow{-2}{*}{DeepLabV3+}& \multirow{-2}{*}{BDD100K (\bbest{reference)}}  & std & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.9}$  & $\stdx{0.6}$  & $\stdx{0.3}$  & $\stdx{2.2}$  & $\stdx{0.2}$  & $\stdx{0.2}$  & $\stdx{0.5}$  & $\stdx{0.1}$  & $\stdx{0.6}$  & $\stdx{2.9}$  & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{1.9}$  & $\stdx{0.0}$  & $\stdx{3.0}$  & $\stdx{3.5}$  & $\stdx{0.3}$ \\[-0.3ex] 

\noalign{\hrule height 2pt}

\end{tabular}
}
\end{table*}



==> tables/results_cityscapes.tex <==
\begin{table*}[t]
\vspace{-4mm}
\caption{Target: Cityscapes. Per-class IoU and global mIoU values are shown. For each row, we report the mean and standard deviation based on three train-test runs. For each column, we highlight the best mean IoU/mIoU per \textbf{sub-block} (bold) and \underline{\textbf{block}} (bold-underlined). Two means are highlighted as best if their difference is $<1$.}
\label{tab:cityscapes_quantitative}
\centering
\setlength{\tabcolsep}{0.9mm} 

\scalebox{0.72}[0.72]{
\begin{tabular}{l|c|c|ccccccccccccccccccc!{\vrule width 1pt}c!{\vrule width 1pt}}

Method & Source & & \rotatebox[origin=c]{90}{\footnotesize Road} & \rotatebox[origin=c]{90}{\footnotesize Sidewalk} & \rotatebox[origin=c]{90}{\footnotesize Building} & \rotatebox[origin=c]{90}{\footnotesize Wall} & \rotatebox[origin=c]{90}{\footnotesize Fence} & \rotatebox[origin=c]{90}{\footnotesize Pole} & \rotatebox[origin=c]{90}{\footnotesize Traffic Light} & \rotatebox[origin=c]{90}{\footnotesize Traffic Sign} & \rotatebox[origin=c]{90}{\footnotesize Vegetation} & \rotatebox[origin=c]{90}{\footnotesize Terrain} & \rotatebox[origin=c]{90}{\footnotesize Sky} & \rotatebox[origin=c]{90}{\footnotesize Person} & \rotatebox[origin=c]{90}{\footnotesize Rider} & \rotatebox[origin=c]{90}{\footnotesize Car} & \rotatebox[origin=c]{90}{\footnotesize Truck} & \rotatebox[origin=c]{90}{\footnotesize Bus} & \rotatebox[origin=c]{90}{\footnotesize Train} & \rotatebox[origin=c]{90}{\footnotesize Motorbike} & \rotatebox[origin=c]{90}{\footnotesize Bike} & mIoU  \\ 

\noalign{\hrule height 2pt}

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV}  & mean & $76.9$  & $27.7$  & $85.0$  & $29.5$  & $34.5$  & $38.2$  & $54.5$  & $21.5$  & $86.8$  & $36.8$  & $84.2$  & $69.9$  & $30.2$  & $79.4$  & $35.5$  & $39.3$  & $18.5$  & $28.3$  & $30.7$  & $47.8$ \\ 
& & std & $\stdx{1.4}$  & $\stdx{3.3}$  & $\stdx{0.2}$  & $\stdx{1.9}$  & $\stdx{3.0}$  & $\stdx{1.0}$  & $\stdx{0.7}$  & $\stdx{3.1}$  & $\stdx{0.6}$  & $\stdx{1.5}$  & $\stdx{0.4}$  & $\stdx{0.6}$  & $\stdx{1.1}$  & $\stdx{7.9}$  & $\stdx{2.4}$  & $\stdx{2.3}$  & $\stdx{9.4}$  & $\stdx{5.2}$  & $\stdx{2.7}$  & $\stdx{1.2}$ \\
\multirow{2}{*}{SegFormer} & \multirow{2}{*}{Synscapes}   & mean & $\bbest{91.9}$  & $\bbest{49.4}$  & $78.9$  & $\bbest{36.4}$  & $29.4$  & $50.3$  & $58.1$  & $61.9$  & $\bbest{86.9}$  & $\bbest{38.1}$  & $84.5$  & $72.2$  & $39.7$  & $89.8$  & $25.1$  & $18.7$  & $16.4$  & $38.9$  & $64.8$  & $54.3$ \\ 
& & std & $\stdx{0.9}$  & $\stdx{2.5}$  & $\stdx{3.0}$  & $\stdx{2.9}$  & $\stdx{3.8}$  & $\stdx{1.0}$  & $\stdx{1.3}$  & $\stdx{1.0}$  & $\stdx{0.7}$  & $\stdx{2.8}$  & $\stdx{3.2}$  & $\stdx{0.8}$  & $\stdx{1.1}$  & $\stdx{0.8}$  & $\stdx{2.0}$  & $\stdx{5.5}$  & $\stdx{0.5}$  & $\stdx{2.8}$  & $\stdx{1.7}$  & $\stdx{1.2}$ \\ 
\multirow{2}{*}{SegFormer} & \multirow{2}{*}{{\thedataset}}   & mean & $89.8$  & $46.1$  & $\bbest{87.3}$  & $21.6$  & $\bbest{47.6}$  & $\bbest{56.4}$  & $\bbest{64.0}$  & $\bbest{69.6}$  & $\bbest{87.2}$  & $32.6$  & $\bbest{88.5}$  & $\bbest{77.2}$  & $\bbest{54.9}$  & $\bbest{93.1}$  & $\bbest{69.1}$  & $\bbest{65.3}$  & $\bbest{28.5}$  & $\bbest{50.0}$  & $\bbest{73.2}$  & $\bbest{63.3}$ \\ 
& & std & $\stdx{0.3}$  & $\stdx{1.1}$  & $\stdx{0.2}$  & $\stdx{5.6}$  & $\stdx{0.7}$  & $\stdx{0.4}$  & $\stdx{0.4}$  & $\stdx{0.6}$  & $\stdx{0.4}$  & $\stdx{3.4}$  & $\stdx{1.0}$  & $\stdx{0.8}$  & $\stdx{0.9}$  & $\stdx{0.4}$  & $\stdx{4.9}$  & $\stdx{3.0}$  & $\stdx{10.2}$  & $\stdx{1.5}$  & $\stdx{0.3}$  & $\stdx{0.7}$ \\  \hline

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV+Synscapes}  & mean & $90.5$  & $50.9$  & $\bbest{89.7}$  & $47.9$  & $47.4$  & $54.0$  & ${65.5}$  & $54.8$  & $\bbest{89.8}$  & ${47.4}$  & $\bbest{92.9}$  & $74.0$  & $37.4$  & $90.6$  & $46.2$  & $64.3$  & $\bbest{61.3}$  & $52.6$  & $62.9$  & $64.2$ \\ 
& & std & $\stdx{1.2}$  & $\stdx{3.0}$  & $\stdx{0.1}$  & $\stdx{2.3}$  & $\stdx{0.7}$  & $\stdx{0.4}$  & $\stdx{0.2}$  & $\stdx{1.9}$  & $\stdx{0.4}$  & $\stdx{2.9}$  & $\stdx{0.2}$  & $\stdx{0.4}$  & $\stdx{3.4}$  & $\stdx{0.5}$  & $\stdx{2.9}$  & $\stdx{1.6}$  & $\stdx{5.8}$  & $\stdx{3.2}$  & $\stdx{2.3}$  & $\stdx{0.8}$ \\

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}   & mean & $\bbest{92.3}$  & $\bbest{57.7}$  & $\bbest{90.3}$  & $\bbest{50.2}$  & $\bbest{53.2}$  & $\bbest{58.1}$  & $\bbest{66.7}$  & $\bbest{67.8}$  & $\bbest{90.0}$  & $\bbest{48.5}$  & $91.0$  & $\bbest{79.8}$  & $\bbest{56.5}$  & $\bbest{93.2}$  & $\bbest{71.3}$  & $\bbest{77.1}$  & $60.3$  & $\bbest{61.4}$  & $\bbest{73.5}$  & $\bbest{70.5}$ \\ 
& & std & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{0.3}$  & $\stdx{0.5}$  & $\stdx{0.9}$  & $\stdx{0.6}$  & $\stdx{0.2}$  & $\stdx{1.2}$  & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{1.2}$  & $\stdx{0.5}$  & $\stdx{1.7}$  & $\stdx{0.6}$  & $\stdx{1.4}$  & $\stdx{2.0}$  & $\stdx{4.7}$  & $\stdx{2.9}$  & $\stdx{0.4}$  & $\stdx{0.4}$ \\  \hline

\multirow{2}{*}{HRDA} & \multirow{2}{*}{GTAV}  & mean & $90.3$  & $32.1$  & $\gbbest{91.1}$  & $\gbbest{60.0}$  & $52.8$  & $58.2$  & $64.7$  & ${71.9}$  & $\gbbest{91.5}$  & $48.2$  & $\gbbest{94.1}$  & $75.0$  & $22.9$  & $94.0$  & ${83.2}$  & $73.4$  & $19.3$  & $65.2$  & $66.5$  & $66.0$ \\ 
\UDAbackbone{(DAFormer*)} & & std & $\stdx{3.8}$  & $\stdx{27.4}$  & $\stdx{0.1}$  & $\stdx{1.3}$  & $\stdx{2.2}$  & $\stdx{1.2}$  & $\stdx{0.2}$  & $\stdx{0.5}$  & $\stdx{0.1}$  & $\stdx{1.3}$  & $\stdx{0.1}$  & $\stdx{2.7}$  & $\stdx{21.0}$  & $\stdx{0.1}$  & $\stdx{0.9}$  & $\stdx{8.2}$  & $\stdx{27.3}$  & $\stdx{0.5}$  & $\stdx{0.7}$  & $\stdx{4.9}$ \\
\multirow{2}{*}{HRDA} & \multirow{2}{*}{Synscapes}  & mean & $\bbest{93.6}$  & $\bbest{70.6}$  & $89.1$  & $45.9$  & $49.5$  & $\gbbest{62.6}$  & $\gbbest{68.5}$  & $64.6$  & $90.5$  & $\bbest{51.7}$  & $\gbbest{95.0}$  & $77.8$  & $39.4$  & $93.5$  & $63.8$  & $47.3$  & $65.3$  & $53.9$  & $\gbbest{76.2}$  & $68.4$ \\ 
\UDAbackbone{(DAFormer*)} & & std & $\stdx{1.1}$  & $\stdx{3.7}$  & $\stdx{1.3}$  & $\stdx{1.7}$  & $\stdx{9.9}$  & $\stdx{0.4}$  & $\stdx{1.1}$  & $\stdx{3.5}$  & $\stdx{0.3}$  & $\stdx{3.3}$  & $\stdx{0.0}$  & $\stdx{0.5}$  & $\stdx{2.5}$  & $\stdx{0.6}$  & $\stdx{3.8}$  & $\stdx{7.2}$  & $\stdx{6.7}$  & $\stdx{10.4}$  & $\stdx{0.2}$  & $\stdx{0.9}$ \\
\multirow{2}{*}{HRDA} & \multirow{2}{*}{{\thedataset}}   & mean & $90.5$  & $56.1$  & $\gbbest{91.5}$  & $\gbbest{60.4}$  & $\gbbest{56.9}$  & $\bbest{61.7}$  & $66.2$  & $\bbest{73.5}$  & $\bbest{90.9}$  & $46.4$  & $\gbbest{94.8}$  & $\gbbest{81.3}$  & $\gbbest{61.2}$  & $\gbbest{95.0}$  & $\gbbest{84.7}$  & $\bbest{76.5}$  & $38.1$  & ${63.9}$  & $\gbbest{75.8}$  & $\bbest{71.9}$ \\ 
\UDAbackbone{(DAFormer*)} & & std & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{1.1}$  & $\stdx{0.6}$  & $\stdx{0.9}$  & $\stdx{0.2}$  & $\stdx{0.2}$  & $\stdx{0.2}$  & $\stdx{2.2}$  & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{3.0}$  & $\stdx{4.8}$  & $\stdx{13.2}$  & $\stdx{1.4}$  & $\stdx{0.4}$  & $\stdx{0.7}$ \\  \hline

\multirow{2}{*}{HRDA} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}   & mean & $\gbbest{97.0}$  & $\gbbest{77.8}$  & $\gbbest{92.0}$  & $59.0$  & $\gbbest{57.0}$  & $\gbbest{63.1}$  & $\gbbest{68.4}$  & $\gbbest{75.3}$  & $\gbbest{91.9}$  & $\gbbest{55.5}$  & $\gbbest{94.9}$  & $\gbbest{81.4}$  & $58.4$  & $\gbbest{94.9}$  & $83.4$  & $\gbbest{88.4}$  & $\gbbest{75.4}$  & $\gbbest{65.7}$  & $\gbbest{76.1}$  & $\gbbest{76.6}$ \\ 
\UDAbackbone{(DAFormer*)} & & std & $\stdx{0.3}$  & $\stdx{1.6}$  & $\stdx{0.1}$  & $\stdx{0.7}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{0.3}$  & $\stdx{0.0}$  & $\stdx{1.1}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{3.0}$  & $\stdx{1.8}$  & $\stdx{3.1}$  & $\stdx{1.5}$  & $\stdx{0.2}$  & $\stdx{0.5}$ \\  [-0.3ex] 
 \hline
\rowcolor{gray!20} &   & mean & ${98.5}$  & ${87.1}$  & ${93.5}$  & ${65.8}$  & ${65.4}$  & ${68.5}$  & ${74.7}$  & ${81.9}$  & ${93.1}$  & ${64.9}$  & ${95.5}$  & ${84.2}$  & ${66.3}$  & ${95.7}$  & ${84.4}$  & ${91.5}$  & ${84.1}$  & ${72.8}$  & ${79.7}$  & ${81.5}$ \\ 
 \rowcolor{gray!20}\multirow{-2}{*}{SegFormer}& \multirow{-2}{*}{Cityscapes (\bbest{reference})}& std & $\stdx{0.0}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{2.6}$  & $\stdx{1.1}$  & $\stdx{0.2}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{0.1}$  & $\stdx{1.3}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.6}$  & $\stdx{0.2}$  & $\stdx{2.5}$  & $\stdx{0.8}$  & $\stdx{1.9}$  & $\stdx{1.0}$  & $\stdx{0.1}$  & $\stdx{0.1}$ \\[-0.3ex] 

\specialrule{.14em}{.2em}{.2em}
 &&&&&&&&&&&&&&&&&&&&&&\\[-3ex]


\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{GTAV}  & mean & $68.7$  & $26.3$  & $71.9$  & $\bbest{29.6}$  & $23.9$  & $33.6$  & $41.4$  & $17.2$  & $83.9$  & ${31.2}$  & $50.3$  & $64.7$  & $25.3$  & $64.8$  & ${30.2}$  & $18.0$  & $0.3$  & $20.3$  & $20.2$  & $38.0$ \\ 
& & std & $\stdx{7.7}$  & $ \stdx{2.7}$  & $\stdx{2.5}$  & $\stdx{2.7}$  & $\stdx{0.5}$  & $\stdx{1.1}$  & $\stdx{0.6}$  & $\stdx{1.4}$  & $\stdx{0.3}$  & $\stdx{2.3}$  & $\stdx{4.9}$  & $\stdx{0.9}$  & $\stdx{3.0}$  & $\stdx{15.7}$  & $\stdx{2.4}$  & $\stdx{3.9}$  & $\stdx{0.1}$  & $\stdx{1.6}$  & $\stdx{5.3}$  & $\stdx{0.6}$ \\ 
\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{Synscapes}  & mean & $85.0$  & $\bbest{42.4}$  & $65.6$  & $23.7$  & $16.7$  & ${47.9}$  & ${52.1}$  & ${56.8}$  & $84.4$  & $28.9$  & $77.2$  & $65.7$  & $28.8$  & $\bbest{86.3}$  & $21.2$  & $10.7$  & $4.0$  & ${37.0}$  & $61.0$  & $47.1$ \\ 
& & std & $\stdx{2.1}$  & $\stdx{1.5}$  & $\stdx{3.5}$  & $\stdx{2.5}$  & $\stdx{3.5}$  & $\stdx{0.7}$  & $\stdx{1.1}$  & $\stdx{1.6}$  & $\stdx{0.2}$  & $\stdx{2.0}$  & $\stdx{2.4}$  & $\stdx{0.7}$  & $\stdx{1.3}$  & $\stdx{1.6}$  & $\stdx{2.5}$  & $\stdx{1.4}$  & $\stdx{0.5}$  & $\stdx{2.3}$  & $\stdx{0.4}$  & $\stdx{1.2}$ \\ 
\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{{\thedataset}}   & mean & $\bbest{86.4}$  & $\bbest{42.7}$  & $\bbest{84.4}$  & $25.4$  & $\bbest{40.4}$  & $\bbest{49.6}$  & $\bbest{54.4}$  & $\bbest{62.4}$  & $\bbest{86.4}$  & $\bbest{32.3}$  & $\bbest{84.7}$  & $\bbest{72.5}$  & $\bbest{51.0}$  & $76.1$  & $\bbest{46.6}$  & $\bbest{54.6}$  & $\bbest{23.2}$  & $\bbest{47.2}$  & $\bbest{69.8}$  & $\bbest{57.4}$ \\  
 & & std & $\stdx{0.6}$  & $\stdx{1.1}$  & $\stdx{0.6}$  & $\stdx{3.8}$  & $\stdx{1.5}$  & $\stdx{0.6}$  & $\stdx{0.6}$  & $\stdx{0.0}$  & $\stdx{0.1}$  & $\stdx{1.4}$  & $\stdx{0.7}$  & $\stdx{0.5}$  & $\stdx{1.1}$  & $\stdx{3.8}$  & $\stdx{3.7}$  & $\stdx{10.9}$  & $\stdx{5.8}$  & $\stdx{1.3}$  & $\stdx{0.3}$  & $\stdx{1.3}$ \\  \hline
 
\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{GTAV+Synscapes}  & mean & $88.8$  & $48.5$  & $85.5$  & $42.7$  & $45.1$  & $51.8$  & $59.4$  & $50.7$  & $\bbest{88.7}$  & $35.8$  & $76.6$  & $71.1$  & $30.1$  & ${90.3}$  & $49.1$  & $67.2$  & $43.6$  & $50.3$  & $57.1$  & $59.6$ \\ 
 & & std & $\stdx{1.4}$  & $\stdx{0.8}$  & $\stdx{0.9}$  & $\stdx{2.9}$  & $\stdx{1.5}$  & $\stdx{0.9}$  & $\stdx{1.2}$  & $\stdx{1.5}$  & $\stdx{0.3}$  & $\stdx{3.3}$  & $\stdx{2.2}$  & $\stdx{0.8}$  & $\stdx{2.1}$  & $\stdx{1.0}$  & $\stdx{2.5}$  & $\stdx{3.5}$  & $\stdx{3.7}$  & $\stdx{2.7}$  & $\stdx{1.8}$  & $\stdx{0.6}$ \\ 
 
\multirow{2}{*}{DeepLabV3+} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}  & mean & $\bbest{90.7}$  & $\bbest{52.3}$  & $\bbest{88.9}$  & $\bbest{48.5}$  & $\bbest{50.6}$  & $\bbest{57.6}$  & $\bbest{63.6}$  & $\bbest{64.7}$  & $\bbest{89.6}$  & $\bbest{44.6}$  & $\bbest{91.6}$  & $\bbest{77.5}$  & $\bbest{54.2}$  & $\bbest{91.8}$  & $\bbest{64.7}$  & $\bbest{75.5}$  & $\bbest{56.5}$  & $\bbest{55.6}$  & $\bbest{71.2}$  & $\bbest{67.9}$ \\  
& & std & $\stdx{0.0}$  & $\stdx{0.5}$  & $\stdx{0.3}$  & $\stdx{1.6}$  & $\stdx{0.8}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{1.3}$  & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{0.2}$  & $\stdx{0.4}$  & $\stdx{0.8}$  & $\stdx{0.4}$  & $\stdx{4.2}$  & $\stdx{3.6}$  & $\stdx{4.8}$  & $\stdx{0.5}$  & $\stdx{0.7}$  & $\stdx{0.7}$ \\ \hline

\multirow{2}{*}{Co-training} & \multirow{2}{*}{GTAV}    & mean & $89.9$  & $50.8$  & $\bbest{89.2}$  & ${39.6}$  & $36.1$  & $52.3$  & $57.0$  & $51.6$  & $89.5$  & $48.2$  & $90.0$  & $72.0$  & $46.9$  & $91.5$  & ${57.2}$  & $57.9$  & $0.0$  & $53.6$  & $64.7$  & $59.9$ \\ 
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{0.0}$  & $\stdx{0.9}$  & $\stdx{0.6}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{0.5}$  & $\stdx{0.1}$  & $\stdx{0.6}$  & $\stdx{0.4}$  & $\stdx{0.4}$  & $\stdx{0.6}$  & $\stdx{0.1}$  & $\stdx{1.9}$  & $\stdx{3.0}$  & $\stdx{0.0}$  & $\stdx{0.8}$  & $\stdx{0.1}$  & $\stdx{0.3}$ \\
\multirow{2}{*}{Co-training} & \multirow{2}{*}{Synscapes}    & mean & $\bbest{91.3}$  & $\bbest{54.6}$  & $82.4$  & $36.7$  & $43.6$  & $\bbest{57.3}$  & $\bbest{64.8}$  & ${69.5}$  & $\gbbest{91.3}$  & $\bbest{51.1}$  & $\gbbest{94.1}$  & $77.3$  & $41.4$  & $\bbest{93.5}$  & $17.2$  & $19.6$  & $1.7$  & $\bbest{60.8}$  & $\gbbest{74.8}$  & $59.1$ \\ 
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.5}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{0.3}$  & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{1.6}$  & $\stdx{0.1}$  & $\stdx{1.1}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.9}$  & $\stdx{0.3}$  & $\stdx{0.1}$ \\ 
\multirow{2}{*}{Co-training} & \multirow{2}{*}{{\thedataset}}    & mean & $\gbbest{91.8}$  & $\bbest{53.9}$  & $\bbest{88.9}$  & $\bbest{40.9}$  & $\bbest{51.2}$  & $\bbest{56.7}$  & $59.4$  & $\bbest{71.3}$  & $90.1$  & $\bbest{51.5}$  & $85.2$  & $\bbest{80.7}$  & $\bbest{60.0}$  & $\gbbest{94.3}$  & $\gbbest{79.4}$  & $\bbest{83.7}$  & $\bbest{62.4}$  & $\bbest{61.7}$  & $72.8$  & $\bbest{70.3}$ \\  
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{0.1}$  & $\stdx{1.1}$  & $\stdx{0.2}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{0.0}$  & $\stdx{0.4}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.5}$  & $\stdx{0.0}$  & $\stdx{1.2}$  & $\stdx{1.1}$  & $\stdx{2.1}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.3}$ \\ \hline

\multirow{2}{*}{Co-training} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}  & mean & $\gbbest{96.8}$  & $\gbbest{76.9}$  & $\gbbest{91.8}$  & $\gbbest{56.4}$  & $\gbbest{58.3}$  & $\gbbest{62.4}$  & $\gbbest{67.4}$  & $\gbbest{75.0}$  & $\gbbest{91.7}$  & $\gbbest{57.2}$  & $\gbbest{94.6}$  & $\gbbest{82.1}$  & $\gbbest{62.0}$  & $\gbbest{94.8}$  & $\gbbest{82.7}$  & $\gbbest{90.0}$  & $\gbbest{76.4}$  & $\gbbest{65.2}$  & $\gbbest{75.0}$  & $\gbbest{76.7}$ \\
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{0.5}$  & $\stdx{0.2}$  & $\stdx{0.4}$  & $\stdx{0.2}$  & $\stdx{0.0}$  & $\stdx{0.3}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{1.1}$  & $\stdx{0.0}$  & $\stdx{1.2}$  & $\stdx{0.5}$  & $\stdx{0.6}$  & $\stdx{0.7}$  & $\stdx{0.2}$  & $\stdx{0.1}$ \\ \hline

\rowcolor{gray!20}  &   & mean & ${98.2}$  & ${85.8}$  & ${93.1}$  & ${58.6}$  & ${64.1}$  & ${66.6}$  & ${71.4}$  & ${80.1}$  & ${92.8}$  & ${66.1}$  & ${95.2}$  & ${83.0}$  & ${63.8}$  & ${95.5}$  & ${79.1}$  & ${89.1}$  & ${83.8}$  & ${70.5}$  & ${78.4}$  & ${79.8}$ \\ 
\rowcolor{gray!20} \multirow{-2}{*}{DeepLabV3+} & \multirow{-2}{*}{Cityscapes (\bbest{reference})} & std & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.7}$  & $\stdx{0.9}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{0.3}$  & $\stdx{0.1}$  & $\stdx{1.0}$  & $\stdx{0.0}$  & $\stdx{0.2}$  & $\stdx{0.5}$  & $\stdx{0.1}$  & $\stdx{1.1}$  & $\stdx{0.8}$  & $\stdx{1.2}$  & $\stdx{0.8}$  & $\stdx{0.1}$  & $\stdx{0.1}$ \\[-0.3ex] 
 
\noalign{\hrule height 2pt}

\end{tabular}
}
\end{table*}



==> tables/results_mapillary.tex <==
\begin{table*}[t]
\vspace{-4mm}
\caption{Analogous to Table \ref{tab:cityscapes_quantitative} but for Mapillary Vistas as target.}
\label{tab:mapillary_quantitative}
\centering
\setlength{\tabcolsep}{0.9mm} 
\scalebox{0.72}[0.72]{
\begin{tabular}{l|c|c|ccccccccccccccccccc!{\vrule width 1pt}c!{\vrule width 1pt}}

Method & Source & & \rotatebox[origin=c]{90}{\footnotesize Road} & \rotatebox[origin=c]{90}{\footnotesize Sidewalk} & \rotatebox[origin=c]{90}{\footnotesize Building} & \rotatebox[origin=c]{90}{\footnotesize Wall} & \rotatebox[origin=c]{90}{\footnotesize Fence} & \rotatebox[origin=c]{90}{\footnotesize Pole} & \rotatebox[origin=c]{90}{\footnotesize Traffic Light} & \rotatebox[origin=c]{90}{\footnotesize Traffic Sign} & \rotatebox[origin=c]{90}{\footnotesize Vegetation} & \rotatebox[origin=c]{90}{\footnotesize Terrain} & \rotatebox[origin=c]{90}{\footnotesize Sky} & \rotatebox[origin=c]{90}{\footnotesize Person} & \rotatebox[origin=c]{90}{\footnotesize Rider} & \rotatebox[origin=c]{90}{\footnotesize Car} & \rotatebox[origin=c]{90}{\footnotesize Truck} & \rotatebox[origin=c]{90}{\footnotesize Bus} & \rotatebox[origin=c]{90}{\footnotesize Train} & \rotatebox[origin=c]{90}{\footnotesize Motorbike} & \rotatebox[origin=c]{90}{\footnotesize Bike} & mIoU  \\ 

\noalign{\hrule height 2pt}

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV}  & mean & $83.3$  & $\bbest{40.2}$  & $\bbest{83.9}$  & $\bbest{32.0}$  & $41.4$  & $43.4$  & $53.1$  & $53.4$  & $77.6$  & $43.1$  & $\gbbest{94.8}$  & $70.1$  & $31.9$  & $86.2$  & ${49.3}$  & $42.0$  & $\bbest{21.1}$  & $43.6$  & $22.3$  & $53.3$ \\  
& & std & $\stdx{1.9}$  & $\stdx{3.1}$  & $\stdx{0.1}$  & $\stdx{1.4}$  & $\stdx{0.8}$  & $\stdx{0.5}$  & $\stdx{1.1}$  & $\stdx{1.7}$  & $\stdx{1.3}$  & $\stdx{3.2}$  & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{1.6}$  & $\stdx{1.4}$  & $\stdx{2.0}$  & $\stdx{5.1}$  & $\stdx{4.5}$  & $\stdx{2.4}$  & $\stdx{0.4}$  & $\stdx{0.8}$ \\ 

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{Synscapes}  & mean & $83.6$  & $39.0$  & $72.1$  & $27.0$  & $26.2$  & $39.1$  & $50.2$  & ${66.8}$  & $\bbest{81.4}$  & $\bbest{49.5}$  & $93.3$  & $64.6$  & $43.8$  & $83.5$  & $30.2$  & $8.6$  & $1.9$  & $49.3$  & ${59.2}$  & $51.0$ \\  
& & std & $\stdx{2.3}$  & $\stdx{3.7}$  & $\stdx{1.0}$  & $\stdx{2.6}$  & $\stdx{3.0}$  & $\stdx{1.8}$  & $\stdx{1.6}$  & $\stdx{0.7}$  & $\stdx{0.8}$  & $\stdx{1.3}$  & $\stdx{0.7}$  & $\stdx{2.0}$  & $\stdx{3.6}$  & $\stdx{2.8}$  & $\stdx{2.2}$  & $\stdx{3.4}$  & $\stdx{1.1}$  & $\stdx{1.7}$  & $\stdx{0.7}$  & $\stdx{0.8}$ \\

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{{\thedataset}}   & mean & $\bbest{88.0}$  & $33.2$  & $73.6$  & $13.5$  & $\bbest{44.5}$  & $\bbest{49.6}$  & $\bbest{59.2}$  & $\bbest{69.2}$  & $80.2$  & $48.2$  & $91.2$  & $\bbest{74.3}$  & $\bbest{55.8}$  & $\bbest{89.3}$  & $\bbest{52.1}$  & $\bbest{52.5}$  & $\bbest{21.0}$  & $\bbest{58.0}$  & $\bbest{64.0}$  & $\bbest{58.8}$ \\   
& & std & $\stdx{0.8}$  & $\stdx{4.6}$  & $\stdx{3.0}$  & $\stdx{2.7}$  & $\stdx{1.4}$  & $\stdx{0.2}$  & $\stdx{0.4}$  & $\stdx{0.4}$  & $\stdx{0.3}$  & $\stdx{0.8}$  & $\stdx{1.8}$  & $\stdx{0.2}$  & $\stdx{4.2}$  & $\stdx{0.3}$  & $\stdx{2.9}$  & $\stdx{6.9}$  & $\stdx{2.5}$  & $\stdx{1.3}$  & $\stdx{1.5}$  & $\stdx{0.3}$ \\   \hline

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV+Synscapes}  & mean & $86.6$  & $46.8$  & $85.7$  & $38.3$  & $46.0$  & $47.5$  & $58.5$  & $60.3$  & $\bbest{79.8}$  & $\bbest{48.2}$  & $\gbbest{95.5}$  & $75.4$  & $51.5$  & $89.2$  & $56.3$  & $56.4$  & $28.8$  & $55.5$  & $55.8$  & $61.2$ \\  
& & std & $\stdx{0.4}$  & $\stdx{1.7}$  & $\stdx{0.1}$  & $\stdx{2.3}$  & $\stdx{1.6}$  & $\stdx{0.6}$  & $\stdx{0.5}$  & $\stdx{1.3}$  & $\stdx{0.8}$  & $\stdx{1.0}$  & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{3.1}$  & $\stdx{0.2}$  & $\stdx{2.4}$  & $\stdx{3.2}$  & $\stdx{8.6}$  & $\stdx{1.8}$  & $\stdx{4.5}$  & $\stdx{0.5}$ \\  

\multirow{2}{*}{SegFormer} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}  & mean & $\bbest{90.1}$  & $\bbest{53.3}$  & $\bbest{86.7}$  & $\bbest{42.2}$  & $\bbest{52.4}$  & $\bbest{51.8}$  & $\bbest{62.3}$  & $\bbest{68.8}$  & $\bbest{80.4}$  & $\bbest{48.3}$  & $\bbest{95.6}$  & $\bbest{77.5}$  & $\bbest{61.1}$  & $\bbest{91.8}$  & $\bbest{68.3}$  & $\bbest{69.6}$  & $\bbest{52.3}$  & $\bbest{59.8}$  & $\bbest{63.6}$  & $\gbbest{67.2}$ \\
& & std & $\stdx{0.8}$  & $\stdx{2.3}$  & $\stdx{0.2}$  & $\stdx{1.0}$  & $\stdx{1.6}$  & $\stdx{0.5}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{0.8}$  & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{0.2}$  & $\stdx{0.2}$  & $\stdx{2.2}$  & $\stdx{3.7}$  & $\stdx{5.1}$  & $\stdx{1.1}$  & $\stdx{0.6}$  & $\stdx{0.6}$ \\   \hline


\multirow{2}{*}{HRDA} & \multirow{2}{*}{GTAV}   & mean & $\bbest{85.5}$  & $\bbest{21.0}$  & $\bbest{86.6}$  & $\bbest{46.0}$  & $35.2$  & $47.3$  & $58.0$  & $62.4$  & $66.0$  & $36.5$  & $92.3$  & $65.0$  & $21.7$  & $89.1$  & $58.7$  & $64.2$  & $5.6$  & $14.8$  & $0.0$  & $50.3$ \\
\UDAbackbone{(DAFormer*)} & & std & $\stdx{0.8}$  & $\stdx{7.0}$  & $\stdx{1.1}$  & $\stdx{0.9}$  & $\stdx{0.9}$  & $\stdx{0.4}$  & $\stdx{1.6}$  & $\stdx{8.1}$  & $\stdx{8.0}$  & $\stdx{13.6}$  & $\stdx{0.1}$  & $\stdx{9.7}$  & $\stdx{18.6}$  & $\stdx{0.8}$  & $\stdx{1.1}$  & $\stdx{5.7}$  & $\stdx{3.9}$  & $\stdx{14.8}$  & $\stdx{0.0}$  & $\stdx{0.3}$ \\ 

\multirow{2}{*}{HRDA} & \multirow{2}{*}{Synscapes}  & mean & $\bbest{84.6}$  & $12.8$  & $74.6$  & $26.1$  & $\bbest{43.4}$  & $46.8$  & $51.0$  & ${65.5}$  & $\gbbest{87.8}$  & $\bbest{42.2}$  & $\bbest{92.8}$  & $68.6$  & $51.3$  & $89.2$  & $56.7$  & $58.0$  & $9.8$  & $55.5$  & $62.3$  & $\bbest{56.8}$ \\
\UDAbackbone{(DAFormer*)} & & std & $\stdx{3.1}$  & $\stdx{12.3}$  & $\stdx{10.1}$  & $\stdx{1.4}$  & $\stdx{3.5}$  & $\stdx{2.7}$  & $\stdx{5.9}$  & $\stdx{1.9}$  & $\stdx{0.7}$  & $\stdx{27.6}$  & $\stdx{6.7}$  & $\stdx{6.2}$  & $\stdx{5.2}$  & $\stdx{1.1}$  & $\stdx{6.6}$  & $\stdx{5.7}$  & $\stdx{5.1}$  & $\stdx{4.1}$  & $\stdx{4.6}$  & $\stdx{5.1}$ \\  

\multirow{2}{*}{HRDA} & \multirow{2}{*}{{\thedataset}} & mean & $80.1$  & $7.2$  & $85.2$  & $7.9$  & $35.0$  & $\bbest{50.0}$  & $\bbest{63.4}$  & $\bbest{74.1}$  & $74.2$  & $0.0$  & $\bbest{93.4}$  & $\bbest{78.4}$  & $\bbest{57.0}$  & $\bbest{90.8}$  & $\bbest{66.4}$  & $\bbest{69.8}$  & $\bbest{29.0}$  & $\bbest{57.8}$  & $\bbest{67.7}$  & $\bbest{57.2}$ \\  
\UDAbackbone{(DAFormer*)} & & std & $\stdx{3.4}$  & $\stdx{9.8}$  & $\stdx{0.3}$  & $\stdx{9.4}$  & $\stdx{10.0}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{0.7}$  & $\stdx{1.7}$  & $\stdx{0.0}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{1.0}$  & $\stdx{0.5}$  & $\stdx{1.4}$  & $\stdx{4.9}$  & $\stdx{16.5}$  & $\stdx{2.0}$  & $\stdx{0.8}$  & $\stdx{1.9}$ \\  \hline

\multirow{2}{*}{HRDA} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}  & mean & $88.3$  & $\gbbest{55.4}$  & $\gbbest{88.4}$  & $\gbbest{49.1}$  & $49.7$  & $\gbbest{52.2}$  & $\gbbest{63.9}$  & $\gbbest{75.9}$  & $\gbbest{86.9}$  & $\gbbest{61.1}$  & $\gbbest{97.2}$  & $\gbbest{78.7}$  & $\gbbest{60.9}$  & $\gbbest{91.7}$  & $\gbbest{71.3}$  & $52.7$  & $44.4$  & $\gbbest{58.9}$  & $65.4$  & $\gbbest{68.0}$ \\  
\UDAbackbone{(DAFormer*)} & & std & $\stdx{4.7}$  & $\stdx{5.1}$  & $\stdx{0.2}$  & $\stdx{1.2}$  & $\stdx{1.2}$  & $\stdx{0.5}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{0.6}$  & $\stdx{0.2}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{2.0}$  & $\stdx{0.1}$  & $\stdx{1.0}$  & $\stdx{31.1}$  & $\stdx{6.0}$  & $\stdx{1.6}$  & $\stdx{0.6}$  & $\stdx{2.2}$ \\ 
 \hline
\rowcolor{gray!20}&  & mean & $96.8$  & $82.1$  & $92.2$  & $60.9$  & $71.0$  & $67.1$  & $73.0$  & $83.3$  & $92.5$  & $75.6$  & $98.7$  & $81.0$  & $64.9$  & $93.9$  & $80.0$  & $87.6$  & $68.2$  & $67.8$  & $73.5$  & $79.5$ \\
\rowcolor{gray!20}  \multirow{-2}{*}{SegFormer} & \multirow{-2}{*}{Mapillary Vistas (\bbest{reference})} & std & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{4.7}$  & $\stdx{1.4}$  & $\stdx{0.8}$  & $\stdx{0.5}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{0.3}$  & $\stdx{0.0}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.6}$  & $\stdx{0.6}$  & $\stdx{4.5}$  & $\stdx{0.4}$  & $\stdx{0.2}$  & $\stdx{0.7}$ \\  [-0.3ex] 

\specialrule{.14em}{.2em}{.2em}
 &&&&&&&&&&&&&&&&&&&&&&\\[-3ex]

\multirow{2}{*}{DeeplabV3+} & \multirow{2}{*}{GTAV}  & mean & $68.4$  & $29.5$  & $55.6$  & $\bbest{18.9}$  & $32.2$  & $34.9$  & $\bbest{46.3}$  & $46.4$  & $75.8$  & $34.3$  & $75.2$  & $\bbest{68.1}$  & $30.8$  & $\bbest{81.0}$  & ${38.7}$  & $12.7$  & ${11.4}$  & $32.1$  & $23.6$  & $43.0$ \\ 
& & std & $\stdx{2.8}$  & $\stdx{1.9}$  & $\stdx{3.7}$  & $\stdx{2.8}$  & $\stdx{0.4}$  & $\stdx{1.9}$  & $\stdx{0.9}$  & $\stdx{1.5}$  & $\stdx{0.6}$  & $\stdx{0.8}$  & $\stdx{3.4}$  & $\stdx{1.0}$  & $\stdx{0.6}$  & $\stdx{1.6}$  & $\stdx{0.5}$  & $\stdx{1.3}$  & $\stdx{3.5}$  & $\stdx{1.0}$  & $\stdx{2.0}$  & $\stdx{1.1}$ \\  

\multirow{2}{*}{DeeplabV3+} & \multirow{2}{*}{Synscapes}   & mean & $67.6$  & $\bbest{30.7}$  & $45.0$  & $10.8$  & $10.2$  & $34.2$  & $38.7$  & $\bbest{56.1}$  & $73.4$  & $\bbest{39.1}$  & $78.7$  & $57.6$  & $35.8$  & $76.8$  & $7.3$  & $4.3$  & $0.2$  & $39.6$  & $\bbest{52.4}$  & $39.9$ \\ 
& & std & $\stdx{1.2}$  & $\stdx{0.8}$  & $\stdx{2.6}$  & $\stdx{0.7}$  & $\stdx{1.1}$  & $\stdx{0.7}$  & $\stdx{1.0}$  & $\stdx{1.2}$  & $\stdx{1.3}$  & $\stdx{0.9}$  & $\stdx{1.4}$  & $\stdx{0.5}$  & $\stdx{1.0}$  & $\stdx{2.2}$  & $\stdx{1.1}$  & $\stdx{0.8}$  & $\stdx{0.0}$  & $\stdx{1.3}$  & $\stdx{1.9}$  & $\stdx{0.4}$ \\ 

\multirow{2}{*}{DeeplabV3+} & \multirow{2}{*}{{\thedataset}}  & mean & $\bbest{78.8}$  & $26.1$  & $\bbest{72.8}$  & $10.4$  & $\bbest{34.2}$  & $\bbest{37.7}$  & $43.3$  & $\bbest{56.3}$  & $\bbest{81.0}$  & $36.1$  & $\bbest{87.8}$  & $\bbest{67.7}$  & $\bbest{46.4}$  & $66.1$  & $\bbest{42.1}$  & $\bbest{33.2}$  & $\bbest{15.3}$  & $\bbest{42.5}$  & $\bbest{52.0}$  & $\bbest{48.9}$ \\ 
& & std & $\stdx{0.6}$  & $\stdx{1.5}$  & $\stdx{1.2}$  & $\stdx{0.9}$  & $\stdx{0.6}$  & $\stdx{0.9}$  & $\stdx{0.7}$  & $\stdx{0.4}$  & $\stdx{0.6}$  & $\stdx{0.9}$  & $\stdx{1.1}$  & $\stdx{0.4}$  & $\stdx{0.6}$  & $\stdx{0.4}$  & $\stdx{0.5}$  & $\stdx{0.7}$  & $\stdx{3.2}$  & $\stdx{0.9}$  & $\stdx{0.3}$  & $\stdx{0.4}$ \\  \hline

\multirow{2}{*}{DeeplabV3+} & \multirow{2}{*}{GTAV+Synscapes} & mean & $72.9$  & $33.3$  & $80.2$  & $24.7$  & $36.5$  & $42.9$  & $57.5$  & $58.0$  & $\bbest{78.3}$  & $41.0$  & $92.6$  & $73.5$  & $39.8$  & $\bbest{87.3}$  & $46.9$  & $43.1$  & $12.1$  & $52.3$  & $48.6$  & $53.8$ \\ 
& & std & $\stdx{2.2}$  & $\stdx{2.1}$  & $\stdx{1.1}$  & $\stdx{4.5}$  & $\stdx{0.7}$  & $\stdx{1.1}$  & $\stdx{0.5}$  & $\stdx{4.3}$  & $\stdx{0.4}$  & $\stdx{2.4}$  & $\stdx{1.2}$  & $\stdx{1.1}$  & $\stdx{0.5}$  & $\stdx{0.9}$  & $\stdx{1.7}$  & $\stdx{2.3}$  & $\stdx{4.7}$  & $\stdx{2.4}$  & $\stdx{1.2}$  & $\stdx{1.4}$ \\ 

\multirow{2}{*}{DeeplabV3+} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}  & mean & $\bbest{86.9}$  & $\bbest{50.9}$  & $\bbest{83.1}$  & $\bbest{32.2}$  & $\bbest{44.7}$  & $\bbest{50.4}$  & $\bbest{59.4}$  & $\bbest{66.8}$  & $\bbest{78.5}$  & $\bbest{43.5}$  & $\bbest{94.4}$  & $\bbest{76.1}$  & $\bbest{52.9}$  & $\bbest{87.9}$  & $\bbest{58.0}$  & $\bbest{61.4}$  & $\bbest{18.5}$  & $\bbest{58.4}$  & $\bbest{65.3}$  & $\bbest{61.5}$ \\ 
& & std & $\stdx{0.7}$  & $\stdx{0.8}$  & $\stdx{0.3}$  & $\stdx{0.5}$  & $\stdx{1.0}$  & $\stdx{0.3}$  & $\stdx{0.6}$  & $\stdx{0.7}$  & $\stdx{0.4}$  & $\stdx{0.5}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{1.1}$  & $\stdx{0.5}$  & $\stdx{1.4}$  & $\stdx{1.8}$  & $\stdx{3.0}$  & $\stdx{1.1}$  & $\stdx{0.4}$  & $\stdx{0.5}$ \\ \hline 

\multirow{2}{*}{Co-training} & \multirow{2}{*}{GTAV}  & mean & $\bbest{88.2}$  & $\bbest{44.2}$  & $\bbest{85.3}$  & $\bbest{31.8}$  & $35.5$  & $\bbest{49.3}$  & $\bbest{58.0}$  & $63.1$  & $75.8$  & $51.2$  & $93.2$  & $\bbest{74.4}$  & $50.6$  & $\bbest{88.7}$  & $51.5$  & $31.3$  & $\bbest{11.8}$  & $46.4$  & $45.9$  & $56.6$ \\ 
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{0.5}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.6}$  & $\stdx{0.3}$  & $\stdx{0.2}$  & $\stdx{1.6}$  & $\stdx{2.5}$  & $\stdx{0.6}$  & $\stdx{0.6}$  & $\stdx{0.3}$ \\ 
\multirow{2}{*}{Co-training} & \multirow{2}{*}{Synscapes}  & mean & $78.0$  & $36.3$  & $73.5$  & $16.9$  & $33.8$  & $\bbest{48.4}$  & $56.0$  & $71.0$  & $\gbbest{86.5}$  & $\bbest{56.6}$  & $\gbbest{96.6}$  & $\bbest{74.4}$  & $38.6$  & $\bbest{88.6}$  & $0.6$  & $18.5$  & $0.2$  & $48.5$  & $59.5$  & $51.7$ \\ 
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.2}$  & $\stdx{0.2}$  & $\stdx{0.0}$  & $\stdx{0.0}$  & $\stdx{0.0}$  & $\stdx{0.2}$  & $\stdx{0.9}$  & $\stdx{0.5}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{0.0}$  & $\stdx{0.1}$  & $\stdx{1.6}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{0.4}$  & $\stdx{0.0}$  & $\stdx{0.2}$ \\
\multirow{2}{*}{Co-training} & \multirow{2}{*}{{\thedataset}}  & mean & $80.0$  & $36.6$  & $84.1$  & $24.5$  & $\bbest{44.5}$  & $47.5$  & $\bbest{58.6}$  & $\bbest{73.3}$  & $83.4$  & $43.1$  & $\gbbest{96.5}$  & $\bbest{74.0}$  & $\gbbest{59.7}$  & $63.4$  & $\bbest{63.5}$  & $\bbest{69.9}$  & $7.8$  & $\bbest{57.2}$  & $\bbest{63.8}$  & $\bbest{59.5}$ \\  
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{0.5}$  & $\stdx{0.9}$  & $\stdx{0.4}$  & $\stdx{1.9}$  & $\stdx{1.5}$  & $\stdx{1.3}$  & $\stdx{1.3}$  & $\stdx{0.2}$  & $\stdx{0.1}$ \\ \hline

\multirow{2}{*}{Co-training} & \multirow{2}{*}{GTAV+Synscapes+{\thedataset}}   & mean & $\gbbest{91.7}$  & $\gbbest{55.2}$  & $\gbbest{87.2}$  & $\gbbest{42.3}$  & $\gbbest{56.1}$  & $\gbbest{54.1}$  & $\gbbest{66.6}$  & $\gbbest{74.7}$  & $\gbbest{86.2}$  & $\gbbest{57.8}$  & $\gbbest{97.1}$  & $\gbbest{79.1}$  & $\gbbest{59.9}$  & $\gbbest{92.6}$  & $\gbbest{70.1}$  & $\gbbest{75.4}$  & $\gbbest{32.0}$  & $\gbbest{61.5}$  & $\gbbest{68.5}$  & $\gbbest{68.8}$ \\ 
\UDAbackbone{(DeepLabV3+)} & & std & $\stdx{0.1}$  & $\stdx{0.6}$  & $\stdx{0.0}$  & $\stdx{0.6}$  & $\stdx{0.1}$  & $\stdx{0.2}$  & $\stdx{0.4}$  & $\stdx{0.1}$  & $\stdx{0.0}$  & $\stdx{0.2}$  & $\stdx{0.0}$  & $\stdx{0.1}$  & $\stdx{0.4}$  & $\stdx{0.0}$  & $\stdx{0.6}$  & $\stdx{0.8}$  & $\stdx{2.7}$  & $\stdx{1.3}$  & $\stdx{0.9}$  & $\stdx{0.2}$ \\ \hline

\rowcolor{gray!20}  &   & mean & ${96.4}$  & ${79.8}$  & ${91.0}$  & ${57.0}$  & ${68.4}$  & ${65.6}$  & ${71.8}$  & ${82.6}$  & ${92.2}$  & ${73.8}$  & ${98.6}$  & ${80.9}$  & ${64.2}$  & ${93.7}$  & ${77.2}$  & ${81.0}$  & ${56.6}$  & ${64.6}$  & ${71.3}$  & ${77.2}$ \\ 
\rowcolor{gray!20} \multirow{-2}{*}{DeeplabV3+}& \multirow{-2}{*}{Mapillary Vistas (\bbest{reference})} & std & $\stdx{0.2}$  & $\stdx{0.9}$  & $\stdx{0.1}$  & $\stdx{0.8}$  & $\stdx{0.2}$  & $\stdx{0.1}$  & $\stdx{0.1}$  & $\stdx{0.3}$  & $\stdx{0.0}$  & $\stdx{0.6}$  & $\stdx{0.0}$  & $\stdx{0.7}$  & $\stdx{1.8}$  & $\stdx{0.2}$  & $\stdx{0.3}$  & $\stdx{1.2}$  & $\stdx{2.9}$  & $\stdx{1.7}$  & $\stdx{1.0}$  & $\stdx{0.4}$ \\
\noalign{\hrule height 2pt}

\end{tabular}
}

\end{table*}
